NTIRE 2026 The 3rd Restore Any Image Model (RAIM) Challenge: Multi-Exposure Image Fusion in Dynamic Scenes (Track 2)

This paper presents NTIRE 2026, the 3rd Restore Any Image Model (RAIM) challenge on multi-exposure image fusion in dynamic scenes. We introduce a benchmark that targets a practical yet difficult HDR imaging setting, where exposure bracketing must be fused under scene motion, illumination variation, and handheld camera jitter. The challenge data contains 100 training sequences with 7 exposure levels and 100 test sequences with 5 exposure levels, reflecting real-world scenarios that frequently cause misalignment and ghosting artefacts. We evaluate submissions with a leaderboard score derived from PSNR, SSIM, and LPIPS, while also considering perceptual quality, efficiency, and reproducibility during the final review. This track attracted 114 participating teams and received 987 submissions. The winning methods significantly improved the ability to remove artifacts from multi-exposure fusion and recover fine details. The dataset and the code of each team can be found at the repository: https://github.com/qulishen/RAIM-HDR.

==> sections/phase.tex <==
\section{Challenge Phases and Submission Rules}
\label{sec:phases}

The challenge follows a staged evaluation pipeline designed to balance open benchmarking, fair comparison, and final reproducibility.

\begin{enumerate}
    \item \textbf{January 23, 2026: Training data release.} The training dataset is officially released to participants, marking the start of the development phase.
    
    \item \textbf{March 9, 2026: Official code collection begins.} Organizers start collecting the code packages required for the final review process.
    
    \item \textbf{March 10, 2026, at 14:00 Beijing Time: Test set release.} The test images for the final competition phases are released to the participants.
    
    \item \textbf{March 11, 2026, at 08:00 Beijing Time: Phase 2 ends \& Final Phase opens.} Online evaluation for Phase 2 is closed, and the submission window for the Final Phase opens on Codabench~\cite{codabench2026raimtrack2}. \textit{Note: Each team is allowed a single final submission only.}
    
    \item \textbf{March 12, 2026, at 23:59 Beijing Time: Final submission deadline.} Participants must submit their final packages, including inference code, model weights, and required scripts.
    
    \item \textbf{March 16, 2026: Reproducibility review deadline.} Organizers complete code integrity checks and local reproducibility verification to ensure results are consistent and no cheating has occurred.
    
    \item \textbf{March 19, 2026: Final results announcement.} The official rankings are published. Only submissions passing the reproducibility and integrity checks are eligible for the final ranking.
\end{enumerate}


